Considering Visualization Example Galleries

Example galleries are often used to teach, document, and advertise visually-focused domain-specific languages and libraries, such as those producing visualizations, diagrams, or webpages. Despite their ubiquity, there is no consensus on the role of "example galleries", let alone what the best practices might be for their creation or curation. To understand gallery meaning and usage, we interviewed the creators (N=11) and users (N=9) of prominent visualization-adjacent tools. From these interviews we synthesized strategies and challenges for gallery curation and management (e.g. weighing the costs/benefits of adding new examples and trade-offs in richness vs ease of use), highlighted the differences between planned and actual gallery usage (e.g. opportunistic reuse vs search-engine optimization), and reflected on parts of the gallery design space not explored (e.g. highlighting the potential of tool assistance). We found that galleries are multi-faceted structures whose form and content are motivated to accommodate different usages--ranging from marketing material to test suite to extended documentation. This work offers a foundation for future support tools by characterizing gallery design and management, as well as by highlighting challenges and opportunities in the space (such as how more diverse galleries make reuse tasks simpler, but complicate upkeep).

==> contents/analysis-how-new.tex <==
\section{Analysis: how do creators make a gallery?} 
\label{sec:gallery-how}
\subsection{Creation and Curation}
% \paraheadd{The origin:}
% Nothing appears from the vacuum. 
% \paraheadd{The process.}
Designing DSLs is an iterative process\am{fowler cite?} where the design space generalizes from examples and the examples illustrate the DSL's possibilities. 
% The initial examples originate from the DSL's structure; the DSL results from its essentiality compared to alternative DSLs.  
% For both task creating a DSL and creating examples, the process starts with formulating the design space and an example. 
Creating examples started from the day-one while formulating the design space: \qtc{then we have some examples of showcasing different things people often want to do. And that's how we actually designed language: we made examples and invert the language $$[from the examples]$$ so that it works with the examples that we designed} (\cxx{Dominik}). 
Additionally, the creators are inspired by other galleries to show that they have the parity of what others can do, as well as the uniqueness. 
Being competitive for market share, \toolName{Plot.ly} reproduces examples from \toolName{ggplot2} and \toolName{Matplotlib}, \qtc{literally saying `do you like this $\toolName{Matplotlib}$ plot and here's exactly how you make it'} (\cxx{Nicholas}).
A new DSL is also a reaction to the flaws (\ie negative space) of its alternatives (\cxx{Ib}), from which the creators collect counter-examples automatically. 

As a DSL phases into the maintenance period from active development, the frequency of adding new examples also slows down. The creators occasionally get inspirations and implement new use cases. Yet more often, enthusiastic users contributed a burst of examples in short period of time as the user base grow (\cxx{Xiaoji}). Another way to create new examples is demand-driven in that multiple users asking about a similar question indicates the need for a new example \cxx{Nicholas, Jeff, Fil}. 
DSL creators and maintainers answer questions by showing examples. And some of the examples become part of the gallery, while others are never revisited by the authors (\cxx{Fil}).

The creators become more selective as more examples are added (\cxx{Matt}), and  they ensure that the difference of a new example from existing ones has a clear target in functionality or learning objectives by carefully designed ordering (\cxx{Jeff}). In general, creators avoid repetitive examples that overwhelm users by the quantity. They keep the examples intriguing while filtering out niche examples that distract users with irrelevant details \cxx{Jeff, Dominik, Josh}. For example, new \toolName{Vega-Lite} examples reuse data source from previous ones when possible to share data domain knowledge across examples (\cxx{Dominik}). When concerned about tradeoffs between the interestingness and effectiveness, \toolName{Plot.ly} chose to include an overwhelming amount of digestible examples. They expect users to locate the specific examples in a webpage by the navigation bar or keyword searching as ways to mitigate. 
\cxx{Ib} also faced the tension between performance and cognitive barrier in an example: \qtc{to make sure they load fast we apply some compression on those datasets, and the example code is no longer easy to understand by the end user. }
In \autoref{sec:analysis}, we discuss more challenges raised in the curation process. 

\synthbox{
\underline{\textbf{Takeaway:}} 
The creators design and implement examples together with the main code. The process is often empirical, and the creators do not have systemic ways to measure whether an indivisual example is good. 
% Not only are galleries motivated as a way of testing (\autoref{sec:gallery-why}), but their creation process also resembles unit testing practices. 
}

\subsection{Tensions and Barriers}
Despite all the incentives (\autoref{sec:gallery-why}), gallery creation and maintenance results in a huge burden for DSL developers. These challenges include coordinating and propagating changes through multiple artifacts of the DSL, and how much resource the creators spend on galleries.  

\paraheadd{Maintaining and coordinating the artifacts. }
There are multiple DSL artifacts around the gallery examples that require coordination, including the gallery examples, core software features, testing suite and the software ecosystem. Actions on any of them would likely cause consequences on another component. Here we focus on the changes either caused by or lead to updating the examples.

% core software and test
One challenge that all the author interviewees expressed is \textbf{maintaining the examples (and the testing) when core software changes}. 
\cxx{Matt} explained that \qtc{maintaining documentation for an open source project is a real drag for the most part}, going on to note that \qtc{every time you do that \/[fixing bugs, updating APIs, \etc \/] you have to go and update the documentation too. So it's like this added layer of work, and it becomes hard to keep things in sync.}
% Anytime the software is updated, some examples might break.
Although most of the creator interviewees have built testing infrastructure around their examples to some extent (\autoref{sec:gallery-why}), they all experienced frustrations having to fix gallery examples upon updating the software. 
% \am{make a comment on this}
Detecting example failures is just the first step to repair them, which can take even more efforts. This indicates interpretability and robustness for the gallery testing against main code changes, and highlights the challenge of maintaining a large amount of examples. 

Manually inspecting each example is a common task before releasing. 
% \qtc{If you have a one-to-one mapping between all your things in your examples and your test cases, along with validation that they are producing the right thing, and you can do that with confidence, if you don't, and typically, it's been a mix where some are and some aren't, you go through the documentation, and you manually and you make sure things are still working as a sanity check before you do a big release.} (\cxx{Jeff}) 
\cxx{Jeff} mentioned going through examples manually as a sanity check before big releases because not all examples have one-to-one mapping to testing and validation. 
\cxx{Carlos} envisioned improving the testing pipeline to better detect the ``silent errors'' (\ie program executes but does not behave as expected): \qtc{I would like every single one of the code examples that we have to not only generate output, but also assert things about the output. \/[...\/] So a much better way to do this would be make a single file from which we render here, and also have the test case and so that if something changes on our review format that breaks this expectation, it shouldn't fail to render the web page.}
\cxx{Josh} reflected on the experience of having to re-implement every example after updating \toolName{Penrose}'s features. Noting that even if everything works well, \qtc{\/[adding more examples\/] adds time to the testing \/[because\/] we run a test suite every time we commit something to the repository} (\cxx{Josh}). 
Software version updates could affect the community examples unless they pinned the version, which may break these examples and confuse the readers who are looking for answers containing code examples on StackOverflow \uxx{5}. 
\cxx{Nicholas} stated that software with a larger and more stable audience such as \toolName{Plot.ly} enforces a stronger commitment for backward compatibility and instead \qtc{treats everything as the documentation problem, because \/[the DSL\/] is pretty hard to evolve}.
% \am{add a comment}
{More recent DSLs under developing are more likely to have major refactoring, requiring more efforts fixing the test and gallery examples. In contrast, more developed and broadly adopted DSLs tend to keep everything as is, which will not break the examples but can cause problems for adding and documenting new features. }


% ecosystem
When examples are added, updated or deleted from the gallery, \textbf{syncing up multiple libraries are necessary for DSLs with a larger ecosystem} (\cxx{Dominik}). For example, when a new example is added to \toolName{Vega-Lite}, it is required to be included in the Vega Editor (\ie online playground). And if there are changes to the example data source, the \texttt{vega-datasets} repository needs to be updated while making sure not to break other examples. 
To alleviate the problem, some of these tools use a monorepo to keep things in sync, which galleries might benefit from similarly. 
% \am{comment, maybe something like highlighting the value of something akin to a monorepo but for galleries. alternatively, maybe just connecting with how some of these tools use a monorepo to keep these things in check}

% \am{take away for this section?}

\paraheadd{Resource constraints. }
% Challenges in creating galleries are not always explicitly stated, but rather indicated by their lower priority compared to other tasks,\am{weak bridge} and therein the lack of resources or motivation to expand and improve galleries.
% \am{preview of findings for subsec?}
Maintenance workload is one aspect to determine how much resource to allocate. 
Resource constraints significantly affect the efforts devoted to the documentation and examples. For example, \toolName{Plot.ly} is the only DSL from our interview that explicitly incorporates Searching Engine Optimization (SEO). In contrast, libraries like \toolName{Seaborn} are just led by few developers on their part-time with \qtc{probably too little time to consider the best things to do with galleries} (\cxx{Nicolas}). Further this can be seen from our survey: \toolName{Plot.ly} has nearly 13 times more examples than \toolName{Seaborn}. 
% \am{Its not clear if this is better for users, but does seem to be a clear consequence of Plotl}
% \am{} It is not clear if this is better for users or not.
A straightforward explanation for this much higher volume is that \toolName{Plot.ly} is the primary product of a for product company.
Yet, this is complicated by \toolName{Deck.Gl}'s relatively svelte gallery, consisting of only 39 examples. \toolName{Deck.Gl} was originally produced at Uber as open source software prior that gradually grew to be key part of the spin-out company Unfolded's (where a number of \toolName{deck.gl}'s maintainers worked) infrastructure.
\cxx{Ib} explained that \qtc{often a new layer $[in \toolName{Deck.GL}]$ is developed by engineers at one company, but then they are generous and they open source it...then suddenly the community has to build an example for that.}
% ---although during that time \toolName{Deck.Gl} had already been moved to a foundation model.  
The role of these external incentives does seem to meaningfully guide the documentation strategy for these libraries, with libraries directly at the center of a product offering likely eliciting a greater degree of developer attention vs tools that are merely part of their infrastructure.
% \am{feel like a comment is necessary}
% , however the specific form of that guidance is not clear.

Creating a gallery is usually easier at the beginning as presenting straightforward use cases that justify the need for new features in a library. 
Although, after developing new features, to implement the corresponding examples they \qtc{have to do all the extra work of actually create a beautiful example or finding a dataset that's public with good license. So sometimes it's just like an extra tax on the work to do it} (\cxx{Ib}).
Further, \textbf{as a gallery grows, it requires a series of careful considerations to select and organize the examples} (\autoref{sec:gallery-how}). 
Additional interface design for the gallery becomes essential for efficient example discovery, but it can introduce more cognitive overhead:  
\qtc{If you have a category or directory or a search, then you have to maintain that. It's another feature to deal with. And it adds complexity to the user experience a little bit, because it's another thing they have to go through in order to get started. So there's no reason to do it till you have to} (\cxx{Josh}).

% \am{take away for this section?}
% \synthbox{
% \underline{\textbf{Takeaway:}} 
% Adding more examples seems less prioritized than other developing activities, especially when the time and human resources are limited. 
% Challenges in creating galleries are not always explicitly stated, but rather indicated by the lack of resources or motivation to expand and improve galleries.
% }

\paraheadd{Evaluation and quality assessment. }
\label{sec: gallery-assess}
\leilani{Have we discussed the benefits of creating galleries for DSL authors by this point? There's the marketing thing but otherwise we don't talk about it much. What do DSL creators get out of gallery making?}\am{+1 seeing a list of goals sould be useful}

Growing a gallery can be extremely demanding without immediately demonstrable benefits.
% , moreover, the benefits are not always immediately distinguishable. 
Moreover, the question of \textit{``how important are the examples compared to other DSL artifacts''} does not have a universal answer.
Moreover, the importance of the examples compared to other DSL artifacts (such as tutorials or API documentation) is ambiguous.

\am{this should go to education} For instance, \cxx{Nicholas} emphasized that \qtc{if it's not in the docs, you may as well not have built it. No one is ever going to use it if it's not in the docs. }
More proactively, \cxx{Carlos} explained that they would shape \toolName{Quarto}'s components around how they present the usage in the documentation; if a feature does not fit well with the narratives they will redesign it to match the concepts behind. 
\am{i dont get this line of logic}On the contrary, as the coordinator of the open-governed \toolName{deck.gl}, \cxx{Ib} questioned that they \qtc{could have spent all that time building new great feature that would attract users.} 
\am{comment}

Many interviewees highlighted \textbf{the difficulty in assessing gallery quality}, especially when isolated from the rest of the documentation.  
For instance, \cxx{Josh} observed that \qtc{It's hard to say how much the current instance of the gallery makes a difference versus just, you know, a small number of examples that are highlighting things. You know, it's very hard to tease out all the different parts of the system.}
\cxx{Nicholas} and \cxx{Fil} noted that they keep track of statistics such as webpage traffic in order to analyze what examples are well-received. 
\cxx{Nicholas} also reached out to people with high scores on StackOverflow asking for what was missing, and looked at discussions on Twitter. 
To that end, most creators monitor StackOverflow (\eg{} \cxx{Nicholas}, \cxx{Carlos}, and \cxx{Fil}), online chat rooms (\eg Slack, discord, \etc) (\eg{} \cxx{Matt}, \cxx{Josh}, \cxx{Dominik}, and \cxx{Fil}), and GitHub issues or discussions (all creators). 
DSL creators empirically construct and evaluate the galleries without standard validation mechanisms, which further diminishes the observed value of having better designed galleries.  
Finding means and metrics to automatically evaluate galleries is mostly unexplored. Kruchten~\etal{}~\cite{kruchten_metrics-based_2023} explore metrics for a particular form of gallery (those comparing and contrasting multiple different DSLs), but measurement of values connected with user utility are unknown.  We highlight this as a research opportunity. 

\synthbox{
\underline{\textbf{Takeaway:}} 
The creators are committed to maintaining existing examples when the core development is finished, and care about how reliable (to the users) and maintainable (to the creators) the galleries are over time. 
Further, galleries become increasingly difficult to maintain as the DSL evolves and the user base grows.
Thus, gallery creators consider the trade-offs of making changes carefully and in light of the continuous burden of maintenance.
These burdens are not limited to industry~\cite{akbaba2023troubling}. As many of these projects arise from research, navigating these burdens is a complex process.
%Every creator has a consistent general structure for decision-making, but the process for different DSLs is not determined. 
}

==> contents/analysis-how.tex <==
\section{Analysis: how do creators make a gallery?} 
\label{sec:gallery-how}
% \subsection{Curation Process}
% \paraheadd{The origin:}
% Nothing appears from the vacuum. 
Designing DSLs is an iterative process\am{fowler cite?} where the design space generalizes from examples and the examples illustrate the DSL's possibilities. 
% The initial examples originate from the DSL's structure; the DSL results from its essentiality compared to alternative DSLs.  
% For both task creating a DSL and creating examples, the process starts with formulating the design space and an example. 
Creating examples started from the day-one while formulating the design space: \qtc{then we have some examples of showcasing different things people often want to do. And that's how we actually designed language: we made examples and invert the language so that it works with the examples that we designed} (\cxx{Dominik}). \am{should this be invent not invert?} \jr{invert, because the tought process seems reversed}
Additionally, the creators are inspired by other galleries to show that they have the parity of what others can do, as well as the uniqueness. 
Being competitive for market share, \toolName{Plot.ly} reproduces examples from \toolName{ggplot2} and \toolName{Matplotlib}, \qtc{literally saying `do you like this $\toolName{Matplotlib}$ plot and here's exactly how you make it'} (\cxx{Nicholas}).
A new DSL is also a reaction to the flaws (\ie negative space) of its alternatives (\cxx{Ib}), from which the creators collect counter-examples automatically. 

As a DSL phases into the maintenance period from active development, the frequency of adding new examples also slows down. The creators occasionally get inspirations and implement new use cases. Yet more often, enthusiastic users contributed a burst of examples in short period of time as the user base grow (\cxx{Xiaoji}). Another way to create new examples is demand-driven in that multiple users asking about a similar question indicates the need for a new example \cxx{Nicholas, Jeff, Fil}. 
DSL creators and maintainers answer questions by showing examples. And some of the examples become part of the gallery, while others are never revisited by the authors (\cxx{Fil}).

The creators become more selective as more examples are added (\cxx{Matt}), and  they ensure that the difference of a new example from existing ones has a clear target in functionality or learning objectives by carefully designed ordering (\cxx{Jeff}). In general, creators avoid repetitive examples that overwhelm users by the quantity. They keep the examples intriguing while filtering out niche examples that distract users with irrelevant details \cxx{Jeff, Dominik, Josh}. For example, new \toolName{Vega-Lite} examples reuse data source from previous ones when possible to share data domain knowledge across examples (\cxx{Dominik}). When concerned about tradeoffs between the interestingness and effectiveness, \toolName{Plot.ly} chose to include an overwhelming amount of digestible examples. They expect users to locate the specific examples in a webpage by the navigation bar or keyword searching as ways to mitigate. 
\cxx{Ib} also faced the tension between performance and cognitive barrier in an example: \qtc{to make sure they load fast we apply some compression on those datasets, and the example code is no longer easy to understand by the end user. }
In \autoref{sec:analysis}, we discuss more challenges raised in the curation process. 

\synthbox{
\underline{\textbf{Takeaway:}} 
The creators design and implement examples together with the main code. The process is often empirical, and the creators do not have systemic ways to measure whether an indivisual example is good. 
% Not only are galleries motivated as a way of testing (\autoref{sec:gallery-why}), but their creation process also resembles unit testing practices. 
}

==> contents/analysis-why.tex <==
\section{Analysis: why are galleries created?} \label{sec:gallery-why}
% We first discuss the purpose and strategies for creating a gallery. 
\am{need some overview of what's happening in this section, its very sudden.}

% \subsection{Roles of Galleries}
The intended use of a gallery influences the gallery design and affordances. 
We summarize the purpose planned by the creators and the roles of gallery in the process of completing tasks for users. 

\paraheadd{Marketing \& advertisement:} 
An example gallery is often the face of the DSL as it may be the first way that users interact with it. 
%An example gallery is the interface when the users interact with the DSL for the first time. 
Rich galleries serve as a marketing vehicle, demonstrating the design space of possibilities for the DSL. 
In this case, galleries help users decide whether to choose the DSL based on what they are trying to accomplish. 
\cxx{Matt} notes that \qtc{I'm sure people come to the site, and probably the first thing that they'll look at, it's like, they'll scroll through the examples and try to see `if I were to try to make something like this? Is this up to my quality standards? Like, is it good enough for me to publish something using this tool?'}
% hopes that the gallery viewers answer ``yes'' to all these questions. 
Towards this goal, several creators noted that they (\cxx{Matt, Josh, Xiaoji}) consider \textit{aesthetics} to be an important factor, and attempt to make examples visually appealing, with  \cxx{Josh} summarizing \qtc{we have other examples that are available in the source code repository in in GitHub for the tool. But they're not as visual appealing or widely useful. So the gallery is intended to be a subset of those that are visually appealing and also representative of the kind of things that we expect our users to want to do}. 

The goal of marketing is universal in galleries we interviewed for, which are public and not for internal use only. 
DSL creators anticipate wide adoption of their tools, be it commercialized software or libraries started as research prototypes. 
Commercialized DSLs such as \toolName{Plot.ly} put in huge efforts to compete for the share of the market. With Search Engine Optimization (SEO) in mind, their goal is to rank at the top when users search for keywords about charting (\eg ``Python scatter plot''). 
\qtc{It's just a sprawling thing where every feature gets an example. It's not really like a showcase, you know, or anything, it's not something that's meant to be browsable as a unit, it's meant to be linked directly to any sort of scroll up and down and optimize for using Command F within a page or Google or our search feature}, \cxx{Nicholas} commented. 
This intended usage pattern affects how their gallery is organized: an extensive set of design variants with descriptive headings are stocked in the same webpage, so that the webpage can be better indexed by search engines.   

\paraheadd{Comparative research: }
Other open sourced libraries (non-profit or academic) attract users in a \am{i dont understand this assertion, isnt plotly explicitly this way? dont many galleries do this? eg altair compares itself with matplotlib in a lot of its promotional materials}non-competitive way. In these cases, their gallery is a demonstration of expressiveness and uniqueness, a signal of development status and evidence of community. 
\qtc{Where things become more apparent is when you start looking across tools. And you see galleries from $\toolName{D3}$ will typically involve lots of visualizations that you can't make with $\toolName{ggplot2}$, or $\toolName{Observable Plot}$ or with $\toolName{Vega-Lite}$, because they target different levels of expressiveness. And so as you start to do some of that sort of comparative research across tools, you will also get a sense} (\cxx{Jeff}).
A single gallery cannot represent the \textit{negative space} of what a DSL cannot achieve, which is usually implied or carried out by the \textit{explanation} documentation. 
However, multiple galleries together help users select a suitable DSL by comparison~\cite{tanzil2024people}. 
% even if they cannot represent the negative space of what the DSL cannot achieve. 
This resonates with the work~\cite{kruchten_metrics-based_2023} by Kruchten (\ie \cxx{Nicholas}) \etal, where they propose evaluating DSL notations through a meta gallery. However, they focused on a small set of charts, in the intersection of the design space all targeted DSLs support, to reflect on the difference between multiple notations. And as a result they overlooked how the negative space for a DSL can be inferred by contrasting with other DSLs. 

\leilani{It seems that negative space can be discussed a bit further here. It feels like an unfinished idea atm.}\am{+1}

\paraheadd{Inspiration:}
Galleries provide ideas for common designs as well as design alternatives by displaying the possibilities. 
Common designs facilitate the brainstorming process since they serve as a cheat sheet that reminds users of best practices. Design alternatives are educational at the same time to encourage users to iterate over and compare different designs. 
Highly customized niche examples (\eg \am{this needs to be described slower}playing Pac Man in \toolName{Vega}) draw users attention and make them more engaged in learning  about the DSL (\cxx{Jeff, Fil}), even if they were added just as \am{who said this? be careful with using quotes in a quote rich context}``a testament to power'' and few people would directly reuse them. 
User-contributed showcases also inspired the creators.
Rather than organize the gallery, \toolName{Quarto} uses it as a repository to showcase how people have been using the DSL: 
\qtc{we want people to see what's possible to build with $\toolName{Quarto}$. And a number of the things that people have built are not things we would ever have considered. There's some very advanced things that people do with styles that are really nice} (\cxx{Carlos}). 
\am{make a comment on this?}

\paraheadd{Opportunistic re-use~\cite{beth_kery_exploring_2017}:}
Some creators believe that the examples are designed to be repurposed since they are showing common use cases. 
In this way, users are expected to copy and paste, and then modify it to meet their needs.  
\qtc{Galleries are just fairly lightweight way to get lots and lots of different programs that show different aspects and different patterns. And hopefully provide good starting points for people to copy and modify. So they don't have to start from scratch} (\cxx{Dominik}), in which the idea is similar to treating examples as templates~\cite{bako_user-driven_2023, mcnutt_integrated_2021}. 
\cxx{Nicholas} was skeptical about the opportunistic re-use in reality for smaller galleries (\eg \toolName{Seaborn}): \qtc{the likelihood that one of these things happens to look like what you're trying to make is pretty low. I mean, the design space for charts is huge, right? I just think that the browsing approach to like, providing this information to users doesn't scale. } 
\am{these dont feel connected}
\jr{trying to connect them:}
Therefore, \toolName{Plot.ly} chooses the bottom-up approach to provide abundant minimal examples aid with searching functions for users to mix and match. 
Although the user feedback he observed was polarizing, \cxx{Nicholas} explicitly expressed his favor to this search-oriented model for example repurposing. 
Locating the target example via scrolling and browsing is too challenging because of \toolName{Plot.ly}'s index structure, compared to searching with keywords. 
Opportunistic re-use is also less likely to be applied to showcases and highly-customized examples since they also require mental decomposition. It introduces another barrier that the users need to understand the code, decompose and extract relevant pieces. 


\paraheadd{Education:}
There is nothing wrong about ``give a man a fish'' when they need it, but is the gallery a good vessel for ``teaching a man how to fish''? 
\cxx{Matt} talked about the first attempt to categorize tutorials out of the \am{??}intermixed showcases: \qtc{at some point, the gallery page just had everything on it and it was becoming unwieldy and the tutorials we thought are very useful for people where we're just kind of buried there amongst things that weren't so like, educational in nature. }
People learn from examples, but \qtc{if you want to teach something, you want a simple example that you know, highlights the thing you're trying to teach. Those kinds of teaching examples are not usually good fits for the gallery because of the visual complexity and, you know, and their applicability to a lot of people}. 
\cxx{Josh} had the same opinion that gallery is not the best place to teach a DSL. 
He argued that \qtc{the main purpose of the galleries is an advertisement, not an explanation or something that people are intended to reuse.}

% \qtc{it's another teaching aid, like some people, you know, they'll look at the things that are most interesting to them. And they might not have all the detail of a tutorial, but they can see how it's constructed and learn how certain things are, you know, are actually achieved in the tools} (\cxx{Jeff}).  
However, the galleries are another teaching-aid that engage more people into exploring the DSL. Although galleries lack of the detail of a tutorial, they allow users to see how things are constructed and how goals are achieved with the DSL (\cxx{Jeff}). Being educational is also intrinsic in the usage of many DSLs, and hence embedded in flavorful examples. For example, \toolName{Penrose} is a platform for diagramming challenging technical concepts, which applies to domains especially in K-12 education; and \cxx{Jeff} sought to have \toolName{Vega} gallery examples to convey useful data facts or mirror historical events. 

\paraheadd{Testing:} 
Examples naturally operate as end-to-end test cases. Compared to unit tests that focus on low-level details that may or may not be exposed to the users as features, they give an opportunity to check how good things work when fused together (\cxx{Jeff}). 
Their existence already helps developers to quickly validate the ideas, as a debugging tool for local development even just via visual inspection (\cxx{Xiaoji}), and uncovers compiler performance issues (\cxx{Matt, Ib}). 
Further, the creators set up testing pipelines for the end-to-end examples. 
\toolName{Penrose} guarantees every example in the repository keep running using continuous integration (\cxx{Josh}). 
\toolName{Vega-Lite} and \toolName{Penrose} programmatically check the SVGs generated from programs to assure consistency throughout the code changes. 
However, manual inspections are still unavoidable and challenging with the existing automation. The changes can be subtle and not visually noticeable (\eg slight changes from \toolName{Penrose}'s layout optimization algorithm), or they can be significantly and still correct by definition. As a result, they require human intervention as part of the testing process. 
Facing a similar issue, \cxx{Carlos} has been working on improving \toolName{Quarto}'s integration tests for silent errors \qtc{to not only generate output, but also assert things about the output.} 
Bridging the gaps between programs and the interfaces they are intended to produce is crucial, and the complexity exacerbates with a more expressive DSL. We discuss more challenges and design opportunities about testing and maintenance in \autoref{sec:gallery-how}.


\am{take away for this setion?}

==> contents/challenges.tex <==
% \section{Challenges and Design Opportunities}
\section{Analysis: What can a gallery be?}
\label{sec:analysis}

We next discuss challenges and design opportunities that we observed during interviews.

\subsection{Creation and Maintenance (to creators)}
\label{sec:maintain}



% \begin{itemize}
%     \item Creating a gallery requires a lot of effort. 
%     \item resources need to be distributed to various components to maximize the outcome. things need to be prioritized, and galleries are not always the most pressing issue. 
%     \item there is no clear signal to help evaluate. how large is the marginal gain? 
%     \begin{itemize}
%         \item usually easier at the beginning and gets harder and harder to add new examples. they introduce additional organizational challenges and make maintenance much harder.
%     \end{itemize}
%     \item assumptions are made by the creators for the users. 
% \end{itemize}

Despite all the incentives (\autoref{sec:gallery-why}), gallery creation and maintenance results in a huge burden for DSL developers. These challenges include coordinating and propagating changes through multiple artifacts of the DSL, as well as the tensions between the creator, the users, and how the creators distribute resources. 

\subsubsection{Coordinating DSL Artifacts}
\label{sec: managing}
There are multiple artifacts in the DSL software around the gallery examples that require coordination, including the gallery examples, core software features, testing suite and the software ecosystem. Actions on any of them would likely cause consequences on another component. Here we focus on the changes either caused by or lead to updating the examples.

% core software and test
One challenge that all the author interviewees expressed is \textbf{maintaining the examples (and the surrounding testing) as core software changes}. 
\cxx{Matt} explained that \qtc{maintaining documentation for an open source project is a real drag for the most part}, going on to note that \qtc{every time you do that \/[fixing bugs, updating APIs, \etc \/] you have to go and update the documentation too. So it's like this added layer of, of work, and it's like, it becomes hard to keep things in sync.}
% Anytime the software is updated, some examples might break.
Although most of the creator interviewees have built testing infrastructure around their examples to some extent (\autoref{sec:gallery-why}), they all experienced frustrations having to fix gallery examples upon updating the software. 
\am{make a comment on this}

Manually inspecting each example is a common task before releasing for the DSLs in the interviews. 
% \qtc{If you have a one-to-one mapping between all your things in your examples and your test cases, along with validation that they are producing the right thing, and you can do that with confidence, if you don't, and typically, it's been a mix where some are and some aren't, you go through the documentation, and you manually and you make sure things are still working as a sanity check before you do a big release.} (\cxx{Jeff}) 
\cxx{Jeff} mentioned going through examples manually as a sanity check before big releases because not all examples have one-to-one mapping to testing and validation. 
\cxx{Carlos} envisioned improving the testing pipeline to better detect the ``silent errors'' (\ie program executes but does not behave as expected): \qtc{I would like every single one of the code examples that we have to not only generate output, but also assert things about the output. \/[...\/] So a much better way to do this would be make a single file from which we render here, and also have the test case and so that if something changes on our review format that breaks this expectation, it shouldn't fail to render the web page.}
\cxx{Josh} reflected on the experience of having to re-implement every example after updating \toolName{Penrose}'s features. Noting that even if everything works well, \qtc{\/[adding more examples\/] adds time to the testing \/[because\/] we run a test suite every time we commit something to the repository} (\cxx{Josh}). 
Software version updates could affect the community examples unless they pinned the version, which may break these examples and confuse the readers who are looking for answers containing code examples on StackOverflow \uxx{3}. 
\cxx{Nicholas} observed that to\am{was this actually a quote?} \qtc{never break anything}, software with a larger and more stable audience such as \toolName{Plot.ly} enforces a stronger commitment for backward compatibility and instead \qtc{treats everything as the documentation problem, because \/[the DSL\/] is pretty hard to evolve}.
\am{add a comment}


% ecosystem
When examples are added, updated or deleted from the gallery, \textbf{syncing up multiple libraries are necessary for DSLs with a larger ecosystem} (\cxx{Dominik}). For example, when a new example is added to \toolName{Vega-Lite}, it is required to be included in the Vega Editor (online playground for \toolName{Vega/Vega-Lite}). And if there are changes to the example data source, the \texttt{vega-datasets} repository needs to be updated while making sure not to break other examples. 
\am{comment, maybe something like highlighting the value of something akin to a monorepo but for galleries. alternatively, maybe just connecting with how some of these tools use a monorepo to keep these things in check}

\am{take away for this section?}

% \subsubsection{Ownership and Responsibility}
\label{sec:resource}
\subsubsection{Resource Constraints}
% gallery design 
Challenges in creating galleries are not always explicitly stated, but rather indicated by their lower priority compared to other tasks,\am{weak bridge} and therein the lack of resources or motivation to expand and improve galleries.
% \am{preview of findings for subsec?}

Resource constraints significantly affect the efforts devoted to the documentation and examples. For example, \toolName{Plot.ly} is the only DSL from our interview that explicitly incorporates Searching Engine Optimization (SEO). In contrast, libraries like \toolName{Seaborn} are just led by few developers on their part-time with too little time to consider the best things to do with galleries. \am{evidence of this from interview} Further this can be seen from our survey: \toolName{Plot.ly} has nearly 13 times more examples than \toolName{Seaborn}. 
% \am{Its not clear if this is better for users, but does seem to be a clear consequence of Plotl}
% \am{} It is not clear if this is better for users or not.
A straightforward explanation for this much higher volume is that \toolName{Plot.ly} is the primary product of a for product company.
Yet, this is complicated by \toolName{Deck.Gl}'s relatively svelte gallery, consisting of only 39 examples. \toolName{Deck.Gl} was originally produced at Uber as open source software prior that gradually grew to be key part of the spin-out company Unfolded's (where a number of \toolName{deck.gl}'s maintainers worked) infrastructure.
% ---although during that time \toolName{Deck.Gl} had already been moved to a foundation model.  
The role of these external incentives does seem to meaningfully guide the documentation strategy for these libraries, with libraries directly at the center of a product offering likely eliciting a greater degree of developer attention vs tools that are merely part of their infrastructure.
\am{feel like a comment is necessary}
% , however the specific form of that guidance is not clear.

Creating a gallery is usually easier at the beginning as presenting straightforward use cases that justify the need for new features in a library. 
Although, after developing new features, to implement the corresponding examples they \qtc{have to do all the extra work of actually create a beautiful example or finding a dataset that's public with good license. So sometimes it's just like an extra tax on the work to do it} (\cxx{Ib}).
Further, \textbf{as a gallery grows, it requires a series of careful considerations to select and organize the examples} (\autoref{sec:gallery-how}). 
Additional interface design for the gallery becomes essential for efficient example discovery, but it can introduce more cognitive overhead:  
\qtc{If you have a category or directory or you have a search, then you have to maintain that. And yeah, it's another feature to deal with. And it adds complexity to the user experience a little bit, because it's another thing they have to go through in order to get started. So there's no reason to do it till you have to} (\cxx{Josh}).

\am{take away for this section?}

\subsubsection{Evaluation and Quality Assessment }
\label{sec: gallery-assess}

\leilani{Have we discussed the benefits of creating galleries for DSL authors by this point? There's the marketing thing but otherwise we don't talk about it much. What do DSL creators get out of gallery making?}\am{+1 seeing a list of goals sould be useful}

Growing a gallery can be extremely demanding without immediately demonstrable benefits.
% , moreover, the benefits are not always immediately distinguishable. 
Moreover, the question of \textit{``how important are the examples compared to other DSL artifacts''} does not have a universal answer.
Moreover, the importance of the examples compared to other DSL artifacts (such as tutorials or API documentation) is ambiguous.

For instance, \cxx{Nicholas} emphasized that \qtc{if it's not in the docs, you may as well not have built it. No one is ever going to use it if it's not in the docs. }
More proactively, \cxx{Carlos} explained that they would shape \toolName{Quarto}'s components around how they present the usage in the documentation; if a feature does not fit well with the narratives they will redesign it to match the concepts behind. 
\am{i dont get this line of logic}On the contrary, as the coordinator of the open-governed \toolName{deck.gl}, \cxx{Ib} questioned that they \qtc{could have spent all that time building new great feature that would attract users.} 
\am{comment}

Many interviewees highlighted \textbf{the difficulty in assessing gallery quality}, especially when isolated from the rest of the documentation.  
For instance, \cxx{Josh} observed that \qtc{It's hard to say how much the current instance of the gallery makes a difference versus just, you know, a small number of examples that are highlighting things. You know, it's very hard to tease out all the different parts of the system.}
\cxx{Nicholas} and \cxx{Fil} noted that they keep track of statistics such as webpage traffic in order to analyze what examples are well-received. 
\cxx{Nicholas} also reached out to people with high scores on StackOverflow asking for what was missing, and looked at discussions on Twitter. 
To that end, most creators monitor StackOverflow (\eg{} \cxx{Nicholas}, \cxx{Carlos}, and \cxx{Fil}), online chat rooms (\eg Slack, discord, \etc) (\eg{} \cxx{Matt}, \cxx{Josh}, \cxx{Dominik}, and \cxx{Fil}), and GitHub issues or discussions (all creators). 
DSL creators empirically construct and evaluate the galleries without standard validation mechanisms, which further diminishes the observed value of having better designed galleries.  
Finding means and metrics to automatically evaluate galleries is mostly unexplored. Kruchten~\etal{}~\cite{kruchten_metrics-based_2023} explore metrics for a particular form of gallery (those comparing and contrasting multiple different DSLs), but measurement of values connected with user utility are unknown.  We highlight this as a research opportunity. 


\synthbox{
\underline{\textbf{Takeaway:}} 
The creators are committed to maintaining existing examples when the core development is finished, and care about how reliable (to the users) and maintainable (to the creators) the galleries are over time. 
Further, galleries become increasingly difficult to maintain as the DSL evolves and the user base grows.
Thus, gallery creators consider the trade-offs of making changes carefully and in light of the continuous burden of maintenance.
These burdens are not limited to industry~\cite{akbaba2023troubling}. As many of these projects arise from research, navigating these burdens is a complex process.
%Every creator has a consistent general structure for decision-making, but the process for different DSLs is not determined. 
}

% \leilani{seems also that a big takeaway is that galleries become increasingly difficult to maintain as the underlyling DSL evolves and the user base grows?}

% \am{+1, would be good to add that the endless burden of maintaince is also reflect in visualization research (per Akbaba \etal{}~\cite{akbaba2023troubling}). As many of these projects arise from research, navigating those burdens is complex}

% \leilani{tried to add to the takeway. feel free to edit.}

\subsection{Role of Community (to creators)}

Next we consider how the shape and desires of the user community defines and shapes the content of the gallery.

\subsubsection{Community Examples}
Open source software (OSS) significantly benefits from interacting with outside contributors. A new use case or example is always a good start to contribute in a non-invasive way. Some libraries, such as \toolName{p5.js}~\cite{p5js} centers users ability to contribute as a central use case of their documentation, and try to make the process of adding to that documentation a welcoming and easy process. 

Encouraging people to submit their own examples sometimes is the main way to expand the collection. After the initial showcases he made on his own, \cxx{Matt} collected more instances via the student projects from a course he taught at University of Washington. He observed that \qtc{Just because it's like if I had to go out and track down every single thing that someone had made, probably we wouldn't have had as many entries into the gallery, which defeats the purpose.} \am{could use some massaging}
\cxx{Jeff}, \cxx{Dominik}, \cxx{Carlos}, and \cxx{Josh} agreed on the efficiency of \am{notation?}``turning the example production problem to a selection problem''. 
For instance, the majority of examples in \toolName{Quarto}'s gallery are provided by the users either by pull requests or links to external repositories. 
Similarly, \toolName{Vega-Lite}'s gallery includes a category called ``Community Examples'' containing links to examples that \cxx{Dominik} described as those that they \qtc{don't want to directly include, or it's so complex and needs a lot of setup}.
\am{maybe comment that this is a place where the notion of showcase sometimes appears}\am{repeats with ealrier stuff}
% \jr{need to find a place for this sentence: }Besides the examples, more experienced users volunteer to answer GitHub issues and some even became part of the team, significantly alleviating the maintenance burden of the original main developers. 

To lower the contributor efforts, DSL creators take actions to make the process seamless  in multiple ways. Guideline for deployment and contribution is common for OSS. 
Most charting DSLs (that are not embedded in a general-purpose language like Python) are shipped with a dedicated online playground for fast prototyping, debugging and sharing. For instance, the editor~\cite{vega-editor} for \toolName{Vega} and \toolName{Vega-Lite} includes a DSL-specific editor that includes special affordances for that DSL, such as debugging~\cite{hoffswell2016visual} and performance~\cite{yang2023vegaprof} tools. 
This editor opens directly from examples in those galleries. 
Similarly, it supports link sharing so that specifications, examples, and demos can be shared amongst its community. To wit, \cxx{Jeff} noted that \qtc{not everything has to be shoehorned into the example gallery. But rather, you can have tools or platforms where there might be curated examples, but then other external examples can come play in the same space}. 
Notebooks such as \toolName{Observable} provide a web-based platform for hosting customized examples written in all sorts of libraries a user can import. \cxx{Fil} mentioned how using \toolName{Observable} reduced the workload for managing the gallery interfaces of \toolName{D3} and \toolName{Observable Plot} since the examples are just links to notebooks. 
% While this may decrease maintainer effort, it may make browsing those galleries more intimidating to less experienced users. 

Making a system seamless inevitably makes it seamless for someone and frictionful for someone else. For instance, moving documentation into notebooks can make that documentation less discoverable (\eg{} for search engines) and potentially more intimidating to users less experienced with notebooks while making it easier to maintain.
Even more, some documentation systems push their users to only ask questions in Discords associated with the project, which may be difficult to discover or intimidating to join. 
Striking a balance between being inviting and easy to maintain is a difficult problem. We suggest that explicitly exposing the seams of the gallery (as in Hengesbach's~\cite{hengesbach2022undoing} related call for visualization seamfulness) may make them more approachable by reducing (what novices might perceive as) the apparent perfection or completion of galleries.
% \am{thats wedded to the community or focus?}

% \am{seamfulness \cite{hengesbach2022undoing}}

Despite the example creation labor being outsourced, the curation and management overhead for quality control (see \autoref{sec:maintain}) still apply to monitoring user-contributed examples. 
\am{it would be good to set up blocks earlier bc its a common and well known gallery in vis community}
\cxx{Jeff} and \cxx{Dominik} imagined an ``unofficial'' community gallery inspired by \toolName{bl.ocks.org} (a defunct Gist viewer for HTML/JavaScript examples): \qtc{there are some other examples in which you can try to grow galleries with some maintenance, but not necessarily they don't have to be specifically managed just by a dedicated, particular tool development team} (\cxx{Dominik}).
\cxx{Dominik} further envisioned a two-tier system where a maintainer can \qtc{check a box} for a community example to promote it into the official gallery; forked versions could be tracked to show more variation. 
While they could ``jump into the swimming pool'' of the non-moderated examples, if users want to master the tool, they might walk through a small curated set of examples one-by-one (\cxx{Jeff}). 
In the extreme, a gallery could evolve into a larger database that enables operations such as searching by key features (\eg all chart examples that use binning) or cross-linking throughout the documentation. However, this may clash with the curation of bespoke experiences that are sometimes intended for galleries---as in \cxx{Jeff}'s vision for the \toolName{Vega} gallery. 
% \am{would be good to reflect on the difference between blocks and these more curated things, like why is blocks not sufficent?}


\synthbox{
\underline{\textbf{Takeaway:}} There are tradeoffs in soliciting examples from the broader community to curate the gallery.
It is difficult to control the quality of examples created by outside contributors, but it is faster and easier to build, what is in essence, a large database of examples with community involvement.
Stronger restriction can guarantee higher example quality that meets DSL author expectations, but may severely reduce the number of community submissions to the gallery.}

\subsubsection{Soliciting Feedback}
The value of receiving user submitted examples goes beyond merely having more examples in the gallery and can be used to improve the tool more generally.


For instance, \cxx{Carlos} encourages \toolName{Quarto} users to explore the features without telling them the best way to do it. This way, the development team can observe how people interact with their tool for potential feature enhancements. 
The distribution of types of user submissions also indicates popular usage scenario, which could drive future development and marketing direction. 
Taking a more direct approach, DSL creators interact with users on social media platforms to answer questions, collect feedback, and they also search for how users review the tool (as in \autoref{sec: gallery-assess}). 

% There are more roles the community serve beyond contributing to new examples. 
% DSL creators interact with users directly on social media platforms to answer questions and collect feedback. 
% Although they devote to teaching people about using \toolName{Quarto}, \cxx{Carlos} encourages the users to explore the features without telling them the best way to do it. This way, the development team can observe how people interact with their tool for potential enhancement. 
% The genre of user submissions also indicate popular usage scenario of the tool. 

\am{this paragraph could be a little clearer}Both the explicit feedback and the use cases submitted provide means to compensate the lack of quality assessment (\autoref{sec: gallery-assess}). 
When they notice users confused about the examples from the issues they post, \cxx{Xiaoji} adds explanation to the \toolName{Deck.gl} examples: \qtc{we know not everyone read those but at least when next time someone asked about it, we can just point them to that page which you know has a better explanation than that someone can come up on spot. \/[In this way,\/] we try to make this code adhere to best practice.} 
However, this evaluation model can be noisy and biased. 
% \qtc{One tough thing about making a page like this is that you don't necessarily get a lot of feedback from people. It's kind of like if you don't hear something you hope it's working}

Not all open-source software has a large enough user base to provide consistent and useful feedback,\am{i like this but could use more detail} and the creators assume everything works well if no one complains. 
At the same time, \qtc{if $$[the docs]$$ do a good job, then people stop asking the questions. And they don't talk to you; they just use the docs}, \cxx{Matt} explained. 
Similarly, \cxx{Carlos} noted that if something is hard to learn, then fewer users will try it, and possibility of receiving a bug report about it will decrease even further. 
\am{could use a bridge}
When people do open GitHub issues asking questions, it can be more frustrating that they misuse the GitHub and pollute the ticket system (\cxx{Fil}). 
They also ask about the same questions over and over again, even if the answers have been pointed out in the documentation. 
In the best scenario, more experienced users might volunteer to answer GitHub issues and some even became part of the team to alleviate the maintenance burden of the original main developers (as happen with \toolName{Altair}), \am{informal}which is not always true in reality. 

\synthbox{
\underline{\textbf{Takeaway:}} 
Collecting feedback from users can be a helpful way to identify rough spots, bugs, or places where the documentation is not clear.
However, fielding this feedback increase the maintenance cost, hindering the chance of resolving other problems more responsively. 
}


\subsection{Gallery usage for DSL users} 
In this section, we discuss the usage scenario with \toolName{Plot.ly}, \toolName{Altair} and \toolName{Vega-Lite}, when and why the users consult the galleries, and their strategies to find relevant examples and accomplish tasks. 

\paraheadd{Adoption.}
Users consider adopting a DSL based on certain qualities that facilitate their specific goals. 
With \toolName{Plot.ly}, \altair{} and \vl{}, the users analyze datasets (\uxx{1,2,4}); present analysis and findings in presentations (\uxx{1,2}), data journals (\uxx{6}) and academic papers (\uxx{1,3,5}); implementing and testing research prototypes (\uxx{1,3}); and teach data science classes (\uxx{1,7}). 
For example, \uxx{2} started exploring \toolName{Plot.ly} after finding a Stack Overflow answer implementing the design they need (Kernel Density plot with zooming). \uxx{3} integrated \toolName{Vega-Lite} in their research pipeline to generate SVG outputs because they contain the required information format. 
The users generally recognized the superiority in the interactions the DSL supports (\uxx{1,2,4,6,7}), ease-of-use (\uxx{1,5-7}), and its popularity (\uxx{2-7}). 
The gallery examples show evidence of these traits when the users encounter them through searching or word of mouth. They demonstrate the possibilities with the visual outputs, and show how they can be efficiently achieved by the accompanying code. 

\paraheadd{When \& why.}
All users interviewed seek to find examples for reuse when they know the target chart type in mind. 
\uxx{1,2,6,7} stated they make charts of common and simple types such as line charts from scratch because it only requires a few lines of code from memory. They refer to the gallery when in need of examples that are \qtu{not the simplest, like anything stacked} (\uxx{6}) and when \qtu{it's just easier to start from something exists than from scratch} (\uxx{3}). 
\vl{}, \altair{} and \plotly{} are less used as inspiration of design ideas because they are high-level DSLs, not designed for highly customized instances. 
However, their galleries are used as a ``cheat sheet'' where the users can get design and implementation hints on spot. \uxx{5} browses the gallery examples looking for additional accessories when they have a base design. \uxx{3} is well-familiar with the gallery and has a mental map of each chart's location, so they can easily jump to the example needed and use it as a starter code. \uxx{4} prefers to view the examples as an aid to iterate over the design they brainstormed: \qtu{so it's more of a learning process...there were visualizations that you did not imagine, but now that you know them makes more sense than the things before. }
When using other lower-level DSLs like \toolName{D3} or \toolName{ggplot2}, they search particularly for customization and fancier designs from external websites such as the \asLink{https://informationisbeautiful.net/}{``information is beautiful''} (a database of graphics and data-visuals) (\uxx{1}) and search engines (\uxx{5}). When using \toolName{D3}, \uxx{5} prefers searching online to the gallery because searching is likely to direct them to Stack Overflow where a lot of questions are directly answered. 

The users interviewed are proficient and accustomed to fixed workflows and data domain, so that design inspiration and brainstorming are not always necessary. They mostly work on the same type of data and context (\uxx{2,6}), receive direct instructions on what to create (\uxx{2,4-6}), or have more similar work to refer (\eg charts in academic papers reporting user study data) (\uxx{1,3,5}). 
Although they recalled to \qtu{figure out what it can and cannot do} (\uxx{2}) and \qtu{learn the visualization vocabulary} (\uxx{1,3,6}) when they started to learn the DSLs.

\paraheadd{How.} 
Expert users we interviewed all have a finely tuned process for sorting through examples and deciding relevant instances. They look at different cues in the environment, such as the example titles and the code structures. Even when they look at unfamiliar galleries, they are capable of interpolating from their experience with other DSLs or programming in general. 
\vl{} and \altair{} users (\uxx{3-6}) browse the galleries when searching for relevant examples, while two of the \plotly{} users (\uxx{2,7}) start from Google searches as expected by the gallery designers. \uxx{3} found the categorization useful for quickly locating the charts, compared to \uxx{6} who is not as conscious but became aware of the organization: \qtu{I feel like I have seen that page a fair amount of time by now. So I kind of know how it's organized. Like, I know that the slightly crazier things are at the bottom. I know that the maps are towards the bottom too. And I know that like basic stacks and stuff like that are higher up at the top. }
\uxx{1} spoke about how they wish there were an additional overview of all variant examples with a \qtu{more scientific} designed arrangement. 
In general, galleries are one of the many tools utilized in each interviewee's customized workflow. 
For instance, \uxx{6} processes data with Pandas, generates the base chart in \toolName{Altair}, and uses Adobe Illustrator to modify the aesthetics and add annotations. \uxx{3} also switches between \toolName{Vega-Lite} and other tools so that he repurposes \toolName{Vega-lite} generated SVGs to the data storytelling usage scenario. In particular, AI-assisted tools are frequently brought up during the interviews.

\jr{feels like the following paragraphs are drifting apart from galleries. but i wanted to talk about using galleries with gpt, and if people replace galleries with gpt then what gpt is better at. }
\uxx{1,2,4,5} mentioned using AI-assisted tools including ChatGPT, Phind and Copilot either in combination with the galleries or as the replacement for specific tasks. 
\uxx{4} first inspects the code recommended by Copilot based on previous code (\eg data manipulation code) or comments. If Copilot could not give a satisfying start code, they would copy an example from the gallery or Stack Overflow, and then modify it with the help of Copilot. \uxx{2} turns to Phind as a replacement of Google searching or Stack Overflow for questions about implementation details.
Framing the Google search queries gets \qtu{progressively and exponentially more difficult}, the more advanced they are in a project when they need to \qtu{get a bit more creative to format the search} (\uxx{2}). With AI-assisted tools, \uxx{2} can \qtu{explain more about what $$[they are]$$ trying to do}, even when they could not figure out a precise query \qtu{as a non-native speaker $$[in English]$$}. 
\uxx{1,5} use ChatGPT similarly for implementation and debugging tasks, and they all developed prompting engineering strategies to fuse into their own workflows. 
The users experienced some well-known limitations with these AI tools. \uxx{5} complained about the model mixing up different versions or hallucinating invalid code, especially for newly developed DSLs with less adoption, and they \qtu{will spend more time on fixing the errors and then realize that the code doesn't work at all.} For the same reason, \uxx{1} choose \toolName{Matplotlib} as the target DSL when using ChatGPT. She also shared lessons-learned from interacting with ChatGPT that suggest using procedural instructions and terms/syntax used by the specific DSL. 

\synthbox{
\underline{\textbf{Takeaway:}} 
Gallery usage behavior can vary based on the specific tasks, users' experience with the notation and supporting tools, and can be affected by how the notations and their galleries are designed. 
Long-term users eventually develope customized workflows that may or may not involve the galleries. 
Frequent gallery users acquire a sense of direction in the gallery with personalized navigation approaches (\eg quickly picking up hints from thumbnails and descriptions). 
}

% In general, AI-powered tools are one component among many other tools, including the galleries, in interviewees' customized workflows. 
% For instance, \uxx{6} processes data with Pandas, generates the base chart in \toolName{Altair}, and uses Adobe Illustrator to modify the aesthetics and add annotations. \uxx{3} also switches between \toolName{Vega-Lite} and other tools so that he repurposes \toolName{Vega-lite} generated SVGs to the data storytelling usage scenario. 

% \paraheadd{Challenges and opportunity. }


\subsection{Communications and Expectations between creators and users}
- hidden assumptions

    - domain knowledge
    
    - data wrangling 
    
    - surrounding environment like react\\
- communication
    
    - ask question effectively
    
    - where to ask questions
    
    - avoid duplicate questions



==> contents/community.tex <==
\section{Analysis: What can a gallery be?}

\subsection{Role of Community (to creators)}

Next we consider how the shape and desires of the user community defines and shapes the content of the gallery.

\subsubsection{Community Examples}
Open source software (OSS) significantly benefits from interacting with outside contributors. A new use case or example is always a good start to contribute in a non-invasive way. Some libraries, such as \toolName{p5.js}~\cite{p5js} centers users ability to contribute as a central use case of their documentation, and try to make the process of adding to that documentation a welcoming and easy process. 

Encouraging people to submit their own examples sometimes is the main way to expand the collection. After the initial showcases he made on his own, \cxx{Matt} collected more instances via the student projects from a course he taught at University of Washington. He observed that \qtc{Just because it's like if I had to go out and track down every single thing that someone had made, probably we wouldn't have had as many entries into the gallery, which defeats the purpose.} \am{could use some massaging}
\cxx{Jeff}, \cxx{Dominik}, \cxx{Carlos}, and \cxx{Josh} agreed on the efficiency of \am{notation?}``turning the example production problem to a selection problem''. 
For instance, the majority of examples in \toolName{Quarto}'s gallery are provided by the users either by pull requests or links to external repositories. 
Similarly, \toolName{Vega-Lite}'s gallery includes a category called ``Community Examples'' containing links to examples that \cxx{Dominik} described as those that they \qtc{don't want to directly include, or it's so complex and needs a lot of setup}.
\am{maybe comment that this is a place where the notion of showcase sometimes appears}\am{repeats with ealrier stuff}
% \jr{need to find a place for this sentence: }Besides the examples, more experienced users volunteer to answer GitHub issues and some even became part of the team, significantly alleviating the maintenance burden of the original main developers. 

To lower the contributor efforts, DSL creators take actions to make the process seamless  in multiple ways. Guideline for deployment and contribution is common for OSS. 
Most charting DSLs (that are not embedded in a general-purpose language like Python) are shipped with a dedicated online playground for fast prototyping, debugging and sharing. For instance, the editor~\cite{vega-editor} for \toolName{Vega} and \toolName{Vega-Lite} includes a DSL-specific editor that includes special affordances for that DSL, such as debugging~\cite{hoffswell2016visual} and performance~\cite{yang2023vegaprof} tools. 
This editor opens directly from examples in those galleries. 
Similarly, it supports link sharing so that specifications, examples, and demos can be shared amongst its community. To wit, \cxx{Jeff} noted that \qtc{not everything has to be shoehorned into the example gallery. But rather, you can have tools or platforms where there might be curated examples, but then other external examples can come play in the same space}. 
Notebooks such as \toolName{Observable} provide a web-based platform for hosting customized examples written in all sorts of libraries a user can import. \cxx{Fil} mentioned how using \toolName{Observable} reduced the workload for managing the gallery interfaces of \toolName{D3} and \toolName{Observable Plot} since the examples are just links to notebooks. 
% While this may decrease maintainer effort, it may make browsing those galleries more intimidating to less experienced users. 

Making a system seamless inevitably makes it seamless for someone and frictionful for someone else. For instance, moving documentation into notebooks can make that documentation less discoverable (\eg{} for search engines) and potentially more intimidating to users less experienced with notebooks while making it easier to maintain.
Even more, some documentation systems push their users to only ask questions in Discords associated with the project, which may be difficult to discover or intimidating to join. 
Striking a balance between being inviting and easy to maintain is a difficult problem. We suggest that explicitly exposing the seams of the gallery (as in Hengesbach's~\cite{hengesbach2022undoing} related call for visualization seamfulness) may make them more approachable by reducing (what novices might perceive as) the apparent perfection or completion of galleries.
% \am{thats wedded to the community or focus?}

% \am{seamfulness \cite{hengesbach2022undoing}}

Despite the example creation labor being outsourced, the curation and management overhead for quality control (see \autoref{sec:gallery-how}) still apply to monitoring user-contributed examples. 
\am{it would be good to set up blocks earlier bc its a common and well known gallery in vis community}
\cxx{Jeff} and \cxx{Dominik} imagined an ``unofficial'' community gallery inspired by \toolName{bl.ocks.org} (a defunct Gist viewer for HTML/JavaScript examples): \qtc{there are some other examples in which you can try to grow galleries with some maintenance, but not necessarily they don't have to be specifically managed just by a dedicated, particular tool development team} (\cxx{Dominik}).
\cxx{Dominik} further envisioned a two-tier system where a maintainer can \qtc{check a box} for a community example to promote it into the official gallery; forked versions could be tracked to show more variation. 
While they could ``jump into the swimming pool'' of the non-moderated examples, if users want to master the tool, they might walk through a small curated set of examples one-by-one (\cxx{Jeff}). 
In the extreme, a gallery could evolve into a larger database that enables operations such as searching by key features (\eg all chart examples that use binning) or cross-linking throughout the documentation. However, this may clash with the curation of bespoke experiences that are sometimes intended for galleries---as in \cxx{Jeff}'s vision for the \toolName{Vega} gallery. 
% \am{would be good to reflect on the difference between blocks and these more curated things, like why is blocks not sufficent?}


\synthbox{
\underline{\textbf{Takeaway:}} There are tradeoffs in soliciting examples from the broader community to curate the gallery.
It is difficult to control the quality of examples created by outside contributors, but it is faster and easier to build, what is in essence, a large database of examples with community involvement.
Stronger restriction can guarantee higher example quality that meets DSL author expectations, but may severely reduce the number of community submissions to the gallery.}

\subsubsection{Soliciting Feedback}
The value of receiving user submitted examples goes beyond merely having more examples in the gallery and can be used to improve the tool more generally.


For instance, \cxx{Carlos} encourages \toolName{Quarto} users to explore the features without telling them the best way to do it. This way, the development team can observe how people interact with their tool for potential feature enhancements. 
The distribution of types of user submissions also indicates popular usage scenario, which could drive future development and marketing direction. 
Taking a more direct approach, DSL creators interact with users on social media platforms to answer questions, collect feedback, and they also search for how users review the tool (as in \autoref{sec: gallery-assess}). 

% There are more roles the community serve beyond contributing to new examples. 
% DSL creators interact with users directly on social media platforms to answer questions and collect feedback. 
% Although they devote to teaching people about using \toolName{Quarto}, \cxx{Carlos} encourages the users to explore the features without telling them the best way to do it. This way, the development team can observe how people interact with their tool for potential enhancement. 
% The genre of user submissions also indicate popular usage scenario of the tool. 

\am{this paragraph could be a little clearer}Both the explicit feedback and the use cases submitted provide means to compensate the lack of quality assessment (\autoref{sec: gallery-assess}). 
When they notice users confused about the examples from the issues they post, \cxx{Xiaoji} adds explanation to the \toolName{Deck.gl} examples: \qtc{we know not everyone read those but at least when next time someone asked about it, we can just point them to that page which you know has a better explanation than that someone can come up on spot. \/[In this way,\/] we try to make this code adhere to best practice.} 
However, this evaluation model can be noisy and biased. 
% \qtc{One tough thing about making a page like this is that you don't necessarily get a lot of feedback from people. It's kind of like if you don't hear something you hope it's working}

Not all open-source software has a large enough user base to provide consistent and useful feedback,\am{i like this but could use more detail} and the creators assume everything works well if no one complains. 
At the same time, \qtc{if $$[the docs]$$ do a good job, then people stop asking the questions. And they don't talk to you; they just use the docs}, \cxx{Matt} explained. 
Similarly, \cxx{Carlos} noted that if something is hard to learn, then fewer users will try it, and possibility of receiving a bug report about it will decrease even further. 
\am{could use a bridge}
When people do open GitHub issues asking questions, it can be more frustrating that they misuse the GitHub and pollute the ticket system (\cxx{Fil}). 
They also ask about the same questions over and over again, even if the answers have been pointed out in the documentation. 
In the best scenario, more experienced users might volunteer to answer GitHub issues and some even became part of the team to alleviate the maintenance burden of the original main developers (as happen with \toolName{Altair}), \am{informal}which is not always true in reality. 

\synthbox{
\underline{\textbf{Takeaway:}} 
Collecting feedback from users can be a helpful way to identify rough spots, bugs, or places where the documentation is not clear.
However, fielding this feedback increase the maintenance cost, hindering the chance of resolving other problems more responsively. 
}


\subsection{Gallery usage for DSL users}
\label{sec: user}
In this section, we discuss the usage scenario with \toolName{Plot.ly}, \toolName{Altair} and \toolName{Vega-Lite}, when and why the users consult the galleries, and their strategies to find relevant examples and accomplish tasks. 

\paraheadd{Adoption.}
Users consider adopting a DSL based on certain qualities that facilitate their specific goals. 
With \toolName{Plot.ly}, \altair{} and \vl{}, the users analyze datasets (\uxx{1,2,4}); present analysis and findings in presentations (\uxx{1,2}), data journals (\uxx{6}) and academic papers (\uxx{1,3,5}); implementing and testing research prototypes (\uxx{1,3}); and teach data science classes (\uxx{1,7}). 
For example, \uxx{2} started exploring \toolName{Plot.ly} after finding a Stack Overflow answer implementing the design they need (Kernel Density plot with zooming). \uxx{3} integrated \toolName{Vega-Lite} in their research pipeline to generate SVG outputs because they contain the required information format. 
The users generally recognized the superiority in the interactions the DSL supports (\uxx{1,2,4,6,7}), ease-of-use (\uxx{1,5-7}), and its popularity (\uxx{2-7}). 
The gallery examples show evidence of these traits when the users encounter them through searching or word of mouth. They demonstrate the possibilities with the visual outputs, and show how they can be efficiently achieved by the accompanying code. 

\paraheadd{When \& why.}
All users interviewed seek to find examples for reuse when they know the target chart type in mind. 
\uxx{1,2,6,7} stated they make charts of common and simple types such as line charts from scratch because it only requires a few lines of code from memory. They refer to the gallery when in need of examples that are \qtu{not the simplest, like anything stacked} (\uxx{6}) and when \qtu{it's just easier to start from something exists than from scratch} (\uxx{3}). 
\vl{}, \altair{} and \plotly{} are less used as inspiration of design ideas because they are high-level DSLs, not designed for highly customized instances. 
However, their galleries are used as a ``cheat sheet'' where the users can get design and implementation hints on spot. \uxx{5} browses the gallery examples looking for additional accessories when they have a base design. \uxx{3} is well-familiar with the gallery and has a mental map of each chart's location, so they can easily jump to the example needed and use it as a starter code. \uxx{4} prefers to view the examples as an aid to iterate over the design they brainstormed: \qtu{so it's more of a learning process...there were visualizations that you did not imagine, but now that you know them makes more sense than the things before. }
When using other lower-level DSLs like \toolName{D3} or \toolName{ggplot2}, they search particularly for customization and fancier designs from external websites such as the \asLink{https://informationisbeautiful.net/}{``information is beautiful''} (a database of graphics and data-visuals) (\uxx{1}) and search engines (\uxx{5}). When using \toolName{D3}, \uxx{5} prefers searching online to the gallery because searching is likely to direct them to Stack Overflow where a lot of questions are directly answered. 

The users interviewed are proficient and accustomed to fixed workflows and data domain, so that design inspiration and brainstorming are not always necessary. They mostly work on the same type of data and context (\uxx{2,6}), receive direct instructions on what to create (\uxx{2,4-6}), or have more similar work to refer (\eg charts in academic papers reporting user study data) (\uxx{1,3,5}). 
Although they recalled to \qtu{figure out what it can and cannot do} (\uxx{2}) and \qtu{learn the visualization vocabulary} (\uxx{1,3,6}) when they started to learn the DSLs.

\paraheadd{How.} 
Expert users we interviewed all have a finely tuned process for sorting through examples and deciding relevant instances. They look at different cues in the environment, such as the example titles and the code structures. Even when they look at unfamiliar galleries, they are capable of interpolating from their experience with other DSLs or programming in general. 
\vl{} and \altair{} users (\uxx{3-6}) browse the galleries when searching for relevant examples, while two of the \plotly{} users (\uxx{2,7}) start from Google searches as expected by the gallery designers. \uxx{3} found the categorization useful for quickly locating the charts, compared to \uxx{6} who is not as conscious but became aware of the organization: \qtu{I feel like I have seen that page a fair amount of time by now. So I kind of know how it's organized. Like, I know that the slightly crazier things are at the bottom. I know that the maps are towards the bottom too. And I know that like basic stacks and stuff like that are higher up at the top. }
\uxx{1} spoke about how they wish there were an additional overview of all variant examples with a \qtu{more scientific} designed arrangement. 
In general, galleries are one of the many tools utilized in each interviewee's customized workflow. 
For instance, \uxx{6} processes data with Pandas, generates the base chart in \toolName{Altair}, and uses Adobe Illustrator to modify the aesthetics and add annotations. \uxx{3} also switches between \toolName{Vega-Lite} and other tools so that he repurposes \toolName{Vega-lite} generated SVGs to the data storytelling usage scenario. In particular, AI-assisted tools are frequently brought up during the interviews.

\jr{feels like the following paragraphs are drifting apart from galleries. but i wanted to talk about using galleries with gpt, and if people replace galleries with gpt then what gpt is better at. }
\uxx{1,2,4,5} mentioned using AI-assisted tools including ChatGPT, Phind and Copilot either in combination with the galleries or as the replacement for specific tasks. 
\uxx{4} first inspects the code recommended by Copilot based on previous code (\eg data manipulation code) or comments. If Copilot could not give a satisfying start code, they would copy an example from the gallery or Stack Overflow, and then modify it with the help of Copilot. \uxx{2} turns to Phind as a replacement of Google searching or Stack Overflow for questions about implementation details.
Framing the Google search queries gets \qtu{progressively and exponentially more difficult}, the more advanced they are in a project when they need to \qtu{get a bit more creative to format the search} (\uxx{2}). With AI-assisted tools, \uxx{2} can \qtu{explain more about what $$[they are]$$ trying to do}, even when they could not figure out a precise query \qtu{as a non-native speaker $$[in English]$$}. 
\uxx{1,5} use ChatGPT similarly for implementation and debugging tasks, and they all developed prompting engineering strategies to fuse into their own workflows. 
The users experienced some well-known limitations with these AI tools. \uxx{5} complained about the model mixing up different versions or hallucinating invalid code, especially for newly developed DSLs with less adoption, and they \qtu{will spend more time on fixing the errors and then realize that the code doesn't work at all.} For the same reason, \uxx{1} choose \toolName{Matplotlib} as the target DSL when using ChatGPT. She also shared lessons-learned from interacting with ChatGPT that suggest using procedural instructions and terms/syntax used by the specific DSL. 

\synthbox{
\underline{\textbf{Takeaway:}} 
Gallery usage behavior can vary based on the specific tasks, users' experience with the notation and supporting tools, and can be affected by how the notations and their galleries are designed. 
Long-term users eventually develope customized workflows that may or may not involve the galleries. 
Frequent gallery users acquire a sense of direction in the gallery with personalized navigation approaches (\eg quickly picking up hints from thumbnails and descriptions). 
}

% In general, AI-powered tools are one component among many other tools, including the galleries, in interviewees' customized workflows. 
% For instance, \uxx{6} processes data with Pandas, generates the base chart in \toolName{Altair}, and uses Adobe Illustrator to modify the aesthetics and add annotations. \uxx{3} also switches between \toolName{Vega-Lite} and other tools so that he repurposes \toolName{Vega-lite} generated SVGs to the data storytelling usage scenario. 

% \paraheadd{Challenges and opportunity. }


\subsection{Communications and Expectations}
% - hidden assumptions

%     - domain knowledge
    
%     - data wrangling 
    
%     - surrounding environment like react\\
% - communication
    
%     - ask question effectively
    
%     - where to ask questions
    
%     - avoid duplicate questions
Although most of these visual DSLs target the broad end users, certain domain knowledge and expertise are expected. 

\subsubsection{Mismatch in expectations}
Visualization languages visually represent data, and often require data wrangling techniques either within the same language (\eg \toolName{Vega}'s data pipeline) or prior to that with external tools (\eg \texttt{pandas} for \toolName{Altair} in Python). Users expressed challenges in integrating multiple tools (\uxx{6}), and spent considerable time adapting data format to visualization specifications (\uxx{1-7}). 

\toolName{Quarto} suffers from a large and diverse set of users with different technical background: \qtc{our examples use \texttt{pandas} because we expect it to be a familiar tool for Python users, but it's a very real problem that we have to guess what's the knowledge base, and have different ways to explain things in code} (\cxx{Carlos}). 
\cxx{Ib} observed the segmentation of community in different groups for developers familiar with functional paradigm, which \toolName{Deck.GL} uses, or imperative programmers. It is intended to be familiar with React users, and can be confusing to the other group. However, \qtc{it's very hard to combine React with an imperative API, which $\toolName{Deck.GL}$ works extremely well with} (\cxx{Ib}). 
Users tend to stick to familiar workflow and programming environment unless the new tools are seamless to adopt (\autoref{sec: user}). 
Porting notations developed in JavaScript to Python wrappers (\eg \toolName{Altair} and \toolName{Plot.ly}) reflects the emergence of data science usage in visualization, in which domain new examples like ``Dendrogram of Hierarchical Clustering'' are added. 
These all highlight documentation accommodating different user types. 


\subsubsection{Communicating knowledge}
Communication barrier exists in both directions of delivering information via documentation and receiving questions and feedback from the users. 
Domain concepts~\cite{thayer_theory_2021} that the notation models, along with the terminology used in documentation, impose a steep learning curve for example searching and reusing (\autoref{sec: user}). 
\qtc{It wasn't super clear, what would you call things. Like do you call things facet and sort of trellises or small multiples or panel charts or lattice? I don't know. So we tended to kind of go with everything, like, make sure we can stick all the keywords in the page.} (\cxx{Nicolas}) Although this behavior might help with \toolName{Plot.ly}'s SEO, it can be confusing to the users. 
LLM-assisted tools bypass this issue with latent context. However, it can only delay the learning process or pass the burden to the community and creators rather than completely avoid it. \qtc{People ask questions to try GPT and then they come to us with code that doesn't work. But they don't understand what it's trying to do. And we have no idea how they come to this code and what they are trying to achieve}, \cxx{Fil} gave an evidence of how using GPT blindly blocks the communication. 

\synthbox{
\underline{\textbf{Takeaway:}} 
Usage patterns and domain knowledge are often treated as hidden assumptions. As different user groups all requesting more information in the documentation, designing a tool to deliver the right information at the right time is demanding. Integrating such tool with galleries might provide opportunities for learning when needed.  
}
